On data skewness, stragglers, and MapReduce progress indicators

We tackle the problem of predicting the performance of MapReduce applications, designing accurate progress indicators that keep programmers informed on the percentage of completed computation time during the execution of a job. Through extensive experiments, we show that state-of-the-art progress indicators (including the one provided by Hadoop) can be seriously harmed by data skewness, load unbalancing, and straggling tasks. This is mainly due to their implicit assumption that the running time depends linearly on the input size. We thus design a novel profile-guided progress indicator, called NearestFit, that operates without the linear hypothesis assumption and exploits a careful combination of nearest neighbor regression and statistical curve fitting techniques. Our theoretical progress model requires fine-grained profile data, that can be very difficult to manage in practice. To overcome this issue, we resort to computing accurate approximations for some of the quantities used in our model through space- and time-efficient data streaming algorithms. We implemented NearestFit on top of Hadoop 2.6.0. An extensive empirical assessment over the Amazon EC2 platform on a variety of real-world benchmarks shows that NearestFit is practical w.r.t. space and time overheads and that its accuracy is generally very good, even in scenarios where competitors incur non-negligible errors and wide prediction fluctuations. Overall, NearestFit significantly improves the current state-of-art on progress analysis for MapReduce.

==> related.tex <==
%!TEX root = MRprof.tex

\section{Related work}
\label{se:related-work}

Designing profiling methodologies able to provide insights into the performance of data-parallel jobs and their scaling properties is extremely difficult. In this section we focus on the class of MapReduce computations, which are the target of this paper. 

HiTune~\cite{HiTune} is a lightweight performance analyzer for Hadoop that allows users to identify application hot-spots and hardware problems. PerfXplain~\cite{perfXplain12} addresses performance debugging by comparing the profiles of different MapReduce jobs: programmers specify performance queries and the tool generates explanations obtained from the analysis of a log of past job executions. Similarly, self-tuning systems such as Starfish~\cite{starfish11} can help users understand and optimize many configuration parameters of Hadoop. With respect to our work, these papers target different goals.

%\paragraph{Performance prediction.} 

A different line of research has addressed the problem of performance prediction in the context of MapReduce-style applications. Accurate predictions can be exploited for different practical purposes, ranging from more precise progress indicators to different optimization strategies able to reduce the job completion time.
Parallax~\cite{parallax} is a progress indicator for MapReduce pipelines based on a linear prediction model similar to {\tt JobRatio}. It can use job profiles collected on past executions. Paratimer~\cite{paratimer} extends Parallax towards workflows characterized by complex DAGs: it can predict the progress of parallel queries by analyzing the critical path in the computation. 
ARIA~\cite{ARIA11} is a framework for automatically allocating the proper amount of cluster resources in order to complete a job within a certain (soft) time deadline. Exploiting job profiles collected on past executions, the linear performance model proposed by ARIA determines the task parallelism sufficient to meet the deadline. To the best of our knowledge (and as shown in this paper), none of these  works is able to  predict accurately the running time of MapReduce applications in presence of both  data skewness and super-linear reduce functions.

%Performance prediction has been exploited also to address the problem of data skewness avoidance and mitigation. 

Uneven data distribution is one of the main reasons for struggler tasks in MapReduce jobs. Several works~\cite{skewtune, Le2014, chisel, Gufler2011} have thus approached this challenge: their main idea is to detect stragglers and split them as soon as possible in order to reduce the job completion time. Akin to this paper, \cite{Gufler2011} considers the problem of super-linear reduce implementations alongside data skewness, but requires a user-defined cost model for predicting the reduce running time. Moreover, the size $|V_k|$ of the key group processed by a reduce function is not collected explicitly, but is estimated as an average among the sizes of all the key groups assigned to the reduce task. Though efficient, this could be rather inaccurate. Load balancing for reduce tasks is also addressed in~\cite{Le2014}, where map outputs are sampled and  the most frequent keys are detected: this is similar to our notion of explicit keys, but we avoid sampling thanks to the use of streaming data structures. 



%A platform-independent metric for measuring the computational complexity of the map and reduce phases is instead proposed in~\cite{Lin2012}, yielding a model which can predict the performance of a job even on heterogeneous clusters. Other systems, such as SkewReduce~\cite{skewreduce}, require instead the user to provide cost functions for accurately modeling the map and reduce running times.




%In the last few years, the problem of performance prediction in the context of MapReduce applications has been targeted by several papers. Indeed, accurate prediction of the running time of MapReduce applications can be exploited for different practical purposes, ranging from more precise progress indicators to different optimization strategies able to reduce the job completion time. 

%Parallax~\cite{parallax} is a progress indicator for MapReduce pipelines that estimates the running time of each job inside the pipeline by multiplying the amount of job input data and an estimated processing speed. Both the input data and the processing speed can be obtained from past executions or derived using online techniques (e.g., by running the job over sampled data). Paratimer~\cite{paratimer} extends Parallax towards workflows characterized by complex DAGs: by analyzing the critical path in the computation, Paratimer is able to accurately predict the progress of parallel queries generated by interfaces such as Pig~\cite{pig08}. 

%ARIA~\cite{ARIA11} is a framework for automatically allocating the proper amount of cluster resources in order to complete a job within a certain (soft) time deadline. Exploiting job profiles collected on past executions, the linear performance model designed by ARIA is able to compute the task parallelism required by a job in order to meet a given deadline. Similarly, \cite{Xie2012} proposed a projection model that can predict the running time of an application when different parameters are scaled (e.g., input data, task parallelism, data locality) by taking benefit of job profiles on past executions. Cherkasova {\em et al.}~\cite{microbench} have shown that the performance of several MapReduce phases (e.g., shuffling) is application-independent, and therefore the running time of these phases can be safely estimated using only execution profiles collected on micro-benchmarks. A platform-independent metric for measuring the computational complexity of the map and reduce phases is instead proposed in~\cite{Lin2012}, yielding a model which can predict the performance of a job even on heterogeneous clusters. Other systems, such as SkewReduce~\cite{skewreduce}, require instead the user to provide cost functions for accurately modeling the map and reduce running times.

%The problem of accurately characterizing the progress of MapReduce jobs in the presence of superlinear map/reduce functions and data skewness has not been targeted by previous works.

%\paragraph{Data skewness.} ...


